A Data Capsule Framework For Web Services: Providing Flexible Data Access Control To Users

This paper introduces the notion of a secure data capsule, which refers to an encapsulation of sensitive user information (such as a credit card number) along with code that implements an interface suitable for the use of such information (such as charging for purchases) by a service (such as an online merchant). In our capsule framework, users provide their data in the form of such capsules to web services rather than raw data. Capsules can be deployed in a variety of ways, either on a trusted third party or the user's own computer or at the service itself, through the use of a variety of hardware or software modules, such as a virtual machine monitor or trusted platform module: the only requirement is that the deployment mechanism must ensure that the user's data is only accessed via the interface sanctioned by the user. The framework further allows an user to specify policies regarding which services or machines may host her capsule, what parties are allowed to access the interface, and with what parameters. The combination of interface restrictions and policy control lets us bound the impact of an attacker who compromises the service to gain access to the user's capsule or a malicious insider at the service itself.

==> prn2eps <==
ps2epsi $1.prn $1.eps
cp -f $1.eps /tmp/$1.eps
cat $1.eps | grep -v "\[Page: 1\]" | grep -v "\[LastPage\]" | grep -v "ProductName:" > /tmp/$1.eps
mv /tmp/$1.eps $1.eps

